Distributed Rate-Splitting Multiple Access for Multilayer Satellite Communications

Future wireless networks, in particular, 5G and beyond, are anticipated to deploy dense Low Earth Orbit (LEO) satellites to provide global coverage and broadband connectivity. However, the limited frequency band and the coexistence of multiple constellations bring new challenges for interference management. In this paper, we propose a robust multilayer interference management scheme for spectrum sharing in heterogeneous satellite networks with statistical channel state information (CSI) at the transmitter (CSIT) and receivers (CSIR). In the proposed scheme, Rate-Splitting Multiple Access (RSMA), as a general and powerful framework for interference management and multiple access strategies, is implemented distributedly at GEO and LEO satellites, coined Distributed-RSMA (D-RSMA). By doing so, D-RSMA aims to mitigate the interference and boost the user fairness of the overall multilayer satellite system. Specifically, we study the problem of jointly optimizing the GEO/LEO precoders and message splits to maximize the minimum rate among User Terminals (UTs) subject to a transmit power constraint at all satellites. A robust algorithm is proposed to solve the original non-convex optimization problem. Numerical results demonstrate the effectiveness and robustness towards network load and CSI uncertainty of our proposed D-RSMA scheme. Benefiting from the interference management capability, D-RSMA provides significant max-min fairness performance gains compared to several benchmark schemes.

==> Formu_Problem/Formulated_prob.tex <==
%Problem formulation
\section{Problem Formulation}\label{sec:Prob_formu}
\par In this section, we focus on designing a joint optimization of \gls{geo}-\gls{leo} beamforming problem that maximizes the minimum fairness rate across all \gls{gus} and \gls{lus} under the constraint of transmit power at all satellites. %For the imperfect \gls{csit} scenario, we maximize worst-case rate. 
% We consider the scenario of \gls{drsma} based multilayer satellite network with perfect \gls{csir} and perfect \gls{csit}.
% with/without satellite channel phase uncertainty.
For \gls{drsma} based multilayer satellite network, the optimization problem can be formulated as
\begin{subequations}\label{prob:formu_prob_orig}
	\begin{align}
		\mathcal{P}_{1}: & \max_{\mathbf{c},\mathbf{W},\mathbf{P}}
		\ \min_{n\in\mathcal{N},k\in\mathcal{K}}\quad  \left\{R_n,R_k\right\}\label{prob:formu_prob_orig_a}                                      \\
		\mbox{s.t.}      & \quad\quad\sum_{n\in\mathcal{N}}C_{g,n}+\sum_{k\in\mathcal{K}}C_{l,k_m}^{sup}\leq R_{c}\label{prob:formu_prob_orig_b} \\
		                 & \quad\quad\sum_{k_m\in\mathcal{K}_m}C_{l,k_m}^{sub}\leq R_{c,m}^{sub},\ m\in\mathcal{M}\label{prob:formu_prob_orig_c} \\
		                 & \quad\quad\mathrm{tr}(\mathbf{W}{\mathbf{W}}^{H})\leq P_g\label{prob:formu_prob_orig_d}                               \\
		                 & \quad\quad\mathrm{tr}(\mathbf{P}_{m}\mathbf{P}_{m}^{H})
		\leq P_l,\ m\in\mathcal{M}\label{prob:formu_prob_orig_e}                                                                                 \\
		                 & \quad\quad\mathbf{c}\succeq\mathbf{0},\label{prob:formu_prob_orig_f}
	\end{align}
\end{subequations}
where $\mathbf{P}=[\mathbf{P}_{1},\ldots,\mathbf{P}_{M}]$ represents the precoding matrix at all \gls{leo} satellites. $\mathbf{c}=[\mathbf{c}_{g},\mathbf{c}_{l}^{sup},\mathbf{c}_{l}^{sub}]$, where $\mathbf{c}_{g}=[C_{g,1},\ldots,C_{g,N}]^T$, $\mathbf{c}_{l}^{sup}=[C_{l,1}^{sup},\ldots,C_{l,K}^{sup}]^T$, and $\mathbf{c}_{l}^{sub}=[C_{l,1}^{sub},\ldots,C_{l,K}^{sub}]^T$ are the vectors of common rate portions. (\ref{prob:formu_prob_orig_b}) ensures that all \gls{gus} and \gls{lus} can successfully decode the common stream $s_{g,c}$. Similarly, (\ref{prob:formu_prob_orig_c}) guarantees that the sub-common stream $s_{l,m}^{sub}$ can be decoded by all \gls{lus} under the coverage of \gls{leo}-$m$. (\ref{prob:formu_prob_orig_d}) and (\ref{prob:formu_prob_orig_e}) represent power constraints of the \gls{geo} and \gls{leo} satellites. (\ref{prob:formu_prob_orig_f}) ensure that all common rate portions are non-negative.



==> System_model/System_model-LAPTOP-S6TTAVLL.tex <==
\section{System model}%\label{sec:System_model}
\par We consider a multilayered satellite system with a single \gls{geo} satellite and $M$ \gls{leo} satellites simultaneously serving $K$ single-antenna \gls{uts}, where $\mathcal{M}=\{1,\ldots,M\}$ and $\mathcal{K}=\{1,\ldots,K\}$. \gls{uts} are divided into $G=M$ groups, and $\mathcal{G}_m$ denote the set of \gls{uts} belonging to the $m$-th \gls{leo} satellite, for all $m\in\mathcal{M}=\{1,\ldots,M\}$. We define the mapping function $\mu(k)=m$%and the inverse mapping function $\mathcal{G}_n=\mu^{-1}(n)$
, $\forall k\in\mathcal{G}_m$. \gls{geo} and \gls{leo} satellites are equipped with $N_t$ feeds array fed reflector antenna and the size of the $m$-th group by $G_m=|\mathcal{G}_m|$. Fig. \ref{fig:sys_illu} shows the system model with $G=M=3$. The coverage of \gls{geo} and \gls{leo} satellites overlaps.

\begin{figure}[b!]
	\centering
	\includegraphics[scale=0.5]{Figures/Illustration_diag.eps}
	\caption{Multilayered satellite system model with $G=3$.}
	\label{fig:sys_illu}
\end{figure}

\par The novel multiple access technique, \gls{rsma}, is distributedly implemented in different satellites, which is denoted as \gls{drsma} in this paper. We demonstrate two structures of \gls{drsma} in this section, named 1-layer \gls{drsma} and a more general and complex one, 2-layer \gls{drsma}.

\subsection{1-layer \gls{drsma}}
We assume that all satellites are served by a same gateway which splits each \gls{ut} message, $W_k$, to a common part, $W_{c,k}$, and a private part, $W_{p,k}$. All common parts are combined and encoded to a common stream, $s_c$, while the private parts are encoded into private streams, $s_k$, for each \gls{ut} independently. We denote the private stream vector for the $m$-th \gls{leo} as $\mathbf{s}_{p,m}=\{s_{k}|k\in\mathcal{G}_m\}$. %, and therefore the total private streams is $\mathbf{s}_{p,L}=\{\mathbf{s}_{p,1},\ldots,\mathbf{s}_{p,M}\}$. 
The common stream is transmitted to \gls{geo} satellite and the private stream vector $\mathbf{s}_{p,m}$ is sent to the corresponding $m$-th \gls{leo} satellite through noiseless feeder links. \gls{geo} satellite broadcasts the common stream to all \gls{uts} and each \gls{leo} transmits using unicast. Hence there is intra-satellite interference between \gls{uts} within each \gls{leo}. The \gls{uts} also receive inter-satellite interference from other \gls{leo} satellites.
\par Data streams are mapped to the transmit antennas via a precoding vector $\mathbf{p}_c$ at \gls{geo} satellite and precoding matrices $\mathbf{P}_{p,m}=\{\mathbf{p}_{k}|k\in\mathcal{G}_m\}$ at $m$-th \gls{leo} satellite, where $\mathbf{p}_c\in\mathbb{C}^{N_t\times1}$, $\mathbf{p}_{k}\in\mathbb{C}^{N_t\times1}$. % and $\mathbf{P}_{p}=\{\mathbf{P}_{p,m}|m\in\mathcal{M}\}$. 
The transmit signals from \gls{geo} and $m$-th \gls{leo} satellite are
\begin{subequations}\label{equ:trans_sig}
	\begin{align}
		 & \mathbf{x}_{G}=\mathbf{p}_cs_c,                    \\
		 & \mathbf{x}_{L,m}=\mathbf{P}_{p,m}\mathbf{s}_{p,m}.
	\end{align}
\end{subequations}
%% Per-antenna feed power constrain
% Because it is difficult to share energy resources among satellite feeds, the transmit power per satellite feed is constrained by $\text{tr}\left(\mathbf{x}_{G}^H\mathbf{x}_{G}\right)\leq\frac{P_{G}}{N_t}$, and $\text{tr}\left(\mathbf{x}_{L,m}^H\mathbf{x}_{L,m}\right)\leq\frac{P_{L}}{N_t}$ for \gls{geo} and \gls{leo} satellite, respectively. 
%% Average power constrain 就假设只有一个beam 
The transmitted signals are subject to the average power constraints, $\mathbb{E}\left\{\mathbf{x}_{G}^H\mathbf{x}_{G}\right\}\leq P_{G}$, and $\mathbb{E}\left\{\mathbf{x}_{L,m}^H\mathbf{x}_{L,m}\right\}\leq P_{L}$.
The signal received at \gls{ut}-$k$ served by the $m$-th \gls{leo} can be expressed as
\begin{equation}\label{equ:received_sig}
	\begin{aligned}
		y_k  =\  & \mathbf{h}^{H}_{G,k} \mathbf{x}_{G}+\sum_{j=1}^M \mathbf{h}_{L,jk}^H\mathbf{P}_{p,j} \mathbf{s}_{p,j}+n_k                                                                 \\
		=\       & \underbrace{\mathbf{h}^{H}_{G,k}\mathbf{p}_{c}s_c+\mathbf{h}^H_{L,mk}\mathbf{p}_{k}s_k}_{\text{Desired signal}}+\underbrace{\mathbf{h}^H_{L,mk}\sum^{G_m}_{\substack{i=1, \\i\neq k}}\mathbf{p}_{i}s_i}_{\text{Intra-\gls{leo} interference}}\\
		         & +\overbrace{\sum^M_{\substack{j=1,                                                                                                                                        \\j\neq m}}\sum^{G_j}_{i=1}\mathbf{h}^H_{L,jk}\mathbf{p}_{i}\mathbf{s}_{i}}^{\text{Inter-\gls{leo} interference}}+n_k,
	\end{aligned}
\end{equation}
where $\mathbf{h}_{G,k}\in\mathbb{C}^{N_t\times1}$ is the channel from the \gls{geo} satellite to \gls{ut}-$k$ %, $\mathbf{H}_{L,m\mathcal{G}_m}\triangleq\left[\mathbf{h}_{L,m1},\ldots,\mathbf{h}_{L,mG_m}\right]$ 
and $\mathbf{h}_{L,jk}\in\mathbb{C}^{N_t\times1}$ is the channel between the $j$-th \gls{leo} satellite and \gls{ut}-$k$, $j\in\mathcal{M}$. $n_k\sim\mathcal{CN}\left(0,\sigma^2_k\right)$ represents the \gls{awgn} at \gls{ut}-$k$. Without loss of generality, the noise variance is assumed as $\sigma^2_k=1,\: \forall k\in\mathcal{K}$.
%\gls{iid} zero-mean\varTheta  complex Gaussian distribution with $\mathbb{E}\left\{\tilde{\mathbf{h}}_{G,k}\tilde{\mathbf{h}}_{G,k}^{H}\right\}=\sigma^2_{Ge,k}\mathbf{I}$. The variance of the error $\sigma^2_{Ge,k}$ is assumed to scale exponentially with SNR as $\sigma^2_{e,k}\sim O(P_{G}^{-\alpha_G})$, where $\alpha_G\in[0,\infty)$ is the quality scaling factor interpreted as the quality of \gls{csit} in the high SNR regime. The scaling factor is truncated such that $\alpha_G\in[0,1]$, in which $\alpha_G=0$ represents partial \gls{csit} with finite precision, e.g. a fixed number of feedback bits, while $\alpha_G=1$ corresponds to perfect \gls{csit}. We assume that the channel between $m$-th \gls{leo} satellite and $k$-th \gls{ut} has similar setting, i.e., $\mathbf{h}_{L,mk}=\hat{\mathbf{h}}_{L,mk}+\tilde{\mathbf{h}}_{L,mk}$, $\mathbb{E}\left\{\tilde{\mathbf{h}}_{L,k}\tilde{\mathbf{h}}_{L,k}^{H}\right\}=\sigma^2_{Le,k}\mathbf{I}$ and $\sigma^2_{e,k}\sim O(P_{L}^{-\alpha_L})$.
\par The intra-\gls{leo} and inter-\gls{leo} interference are handled by \gls{geo} via common stream, because the common message contains a portion of each \gls{ut} message, which means that each \gls{ut} partially decodes the interference and partially treat interference as noise. After each \gls{ut} receives the signal, it first decodes common stream by treating the private streams as noise. The \gls{sinr} of the common stream at \gls{ut}-$k$ served by \gls{leo}-$m$ is
\begin{equation}\label{equ:common_SINR}
	\rho_{c,k}=  \frac{S_{c,k}}{S_{k}+I_{iL,p}+I_{oL,p}+1},
\end{equation}
where $S_{c,k}=|\mathbf{h}^{H}_{G,k}\mathbf{p}_{c}|^2$, $S_{k}=|\mathbf{h}^H_{L,mk}\mathbf{p}_{k}|^2$, $I_{iL,p}=\sum^{G_m}_{i=1,i\neq k}|\mathbf{h}^H_{L,mk}\mathbf{p}_{i}|^2$ and $I_{oL,p}=\sum^M_{j=1,j\neq m}\sum^{G_j}_{i=1}|\mathbf{h}^H_{L,jk}\mathbf{p}_{i}|^2$ denote the power of common stream, the power of designated private stream to \gls{ut}-$k$, the power of private streams for other \gls{uts} from $m$-th \gls{leo} satellite and the power of inter-\gls{leo} interference, respectively. It corresponds to the achievable rate $R_{c,k}=\log_2(1+\rho_{c,k})$. In order to make sure that each \gls{ut} decodes $s_c$, we define the common rate
\begin{equation}
	R_c=\min_{k\in\mathcal{K}}\ R_{c,k}.
\end{equation}
Since the common stream is shared among all \gls{uts}, we define $R_c\triangleq\sum_{k=1}^{K}C_k$, where $C_k$ denotes the $k$-th \gls{ut}'s portion of common rate.
\par Once $s_c$ is decoded, it is subtracted from the received signal. However, perfect \gls{sic} is a unrealistic assumption in the majority of cases, especially in satellite communications. Subsequently, \gls{ut}-$k$ decodes the private stream $s_k$ while treating the other \gls{uts}' private streams as noise. Accordingly,  \gls{ut}-$k$'s decoding of the private stream $s_k$ with imperfect \gls{sic} results in a \gls{sinr} of
\begin{equation}
	\rho_{p,k}=\frac{S_k}{I_{iL,p}+I_{oL,p}+\eta S_{c,k}+1},
\end{equation}
where $\eta\in[0,1]$ is imperfect \gls{sic} parameter. Besides, $0$ and $1$ correspond to the perfect \gls{sic} and not performing \gls{sic}, respectively. The private rate of \gls{ut}-$k$ is expressed as $R_{p,k}=\log_2(1+\rho_{p,k})$. \gls{ut}-$k$ reconstructs the original message after the common and private streams have been decoded by taking the decoded $\widehat{W}_{c,k}$ from the decoded $\widehat{W}_c$ and combining it with the decoded $W_{p,k}$. Therefore, the total transmission rate of \gls{ut}-$k$ is
\begin{equation}\label{equ:1-layer_totoal_rate}
	R_k=C_k+R_{p,k},\ k\in\mathcal{K}.
\end{equation}

\subsection{2-layer \gls{drsma}}
The biggest difference for 2-layer \gls{drsma} lies in the way gateway splits \gls{uts} messages. Each \gls{ut} message, $W_k$, is split into three parts, $\{W_{supc,k}^{\prime},W_{subc,k}^{\prime},W_{p,k}^{\prime}\}$ that corresponds to super common part, sub-common part and private part, respectively. All super common parts are encoded together into a super common stream $s_{supc}^{\prime}$, instead the sub-common parts in which the users belong to the same group (i.e., users are served by the same \gls{leo} satellite) are combined into a sub-common stream, $s_{subc,\mu(k)}^{\prime}$. The private parts are encoded to privates streams, $s_k^{\prime},\,k\in\mathcal{K}$. The super common stream $s_{supc}^{\prime}$ is precoded by precoding vector $\mathbf{p}_c^\prime\in\mathbb{C}^{N_t\times1}$. The sub-common stream from $m$-th \gls{leo} satellite, $s_{subc,m}^{\prime}$ and private streams, $\mathbf{s}_{p,m}^\prime=\{s_k^{\prime}|k\in\mathcal{G}_m\}$, are precoded by precoding vector $\mathbf{p}_{subc,m}^\prime$ and  precoding matrix $\mathbf{P}_{p,m}^\prime=\{\mathbf{p}_{k}^\prime|k\in\mathcal{G}_m\}\in\mathbb{C}^{N_t\times G_m}$, respectively. %The precoding matrix from all \gls{leo} satellites is $\mathbf{P}_{p}^{\prime}=\{\mathbf{P}_{p,m}^{\prime}|m\in\mathcal{M}\}$. 
The transmit signals from \gls{geo} and $m$-th \gls{leo} satellites under 2-layer \gls{drsma} deployment are
\begin{equation}\label{equ:2-layer_trans_sig}
	\begin{aligned}
		 & \mathbf{x}_G^\prime=\mathbf{p}_c^\prime s^\prime_{supc},                                                                \\
		 & \mathbf{x}_{L,m}^\prime=\mathbf{p}_{subc,m}^\prime s_{subc,m}^{\prime}+\mathbf{P}_{p,m}^\prime \mathbf{s}_{p,m}^\prime.
	\end{aligned}
\end{equation}
% where precoding vector $\mathbf{p}_c^\prime\in\mathbb{C}^{N_t\times1}$, precoding matrix $\mathbf{P}_{p,m}^\prime=\{\mathbf{p}_{subc,m}^\prime,\mathbf{p}_{k}^\prime,|k\in\mathcal{G}_m\}\in\mathbb{C}^{N_t\times(G_m+1)}$ and $\mathbf{s}_{p,m}^\prime=\{s_{subc,m}^{\prime},s_k^{\prime}|k\in\mathcal{G}_m\}$. $\mathbf{P}_{p}^{\prime}=\{\mathbf{P}_{p,m}^{\prime}|m\in\mathcal{M}\}$. 
The signal received at \gls{ut}-$k$ under the coverage of \gls{leo}-$m$ is
\begin{equation}\label{equ:2-layer_received_sig}
	\begin{aligned}
		y_k^\prime  =\  & \mathbf{h}^{H}_{G,k}\mathbf{x}_{G}^{\prime}+
		\sum_{j=1}^{M}\mathbf{h}^H_{L,jk}\mathbf{x}_{L,j}^{\prime}+n_k                                                                              \\
		=\              & \mathbf{h}^H_{G,k} \mathbf{p}^\prime_c s^\prime_{supc} + \mathbf{h}^H_{L,mk} \mathbf{p}^\prime_{subc,m} s^\prime_{subc,m} \\
		                & +\sum^{M}_{\substack{j=1,                                                                                                 \\j\neq m}}\mathbf{h}^H_{L,jk} \mathbf{p}^\prime_{subc,j} s^\prime_{subc,j}  + \sum_{i=1}^{G_m} \mathbf{h}^H_{L,mk} \mathbf{p}^\prime_{i} s^\prime_{i} \\
		                & + \sum_{\substack{j=1,                                                                                                    \\j\neq m}}^M\sum_{i=1}^{G_j} \mathbf{h}^H_{L,jk} \mathbf{p}^\prime_{i} s^\prime_{i}+n_k.
	\end{aligned}
\end{equation}
1-layer \gls{drsma} is a subset of 2-layer \gls{drsma}. If the sub-common streams turn off, then 2-layer \gls{drsma} reduces to 1-layer \gls{drsma}.
\par $k$-th \gls{ut} is required to decode three streams $s^\prime_{supc}$, $s^\prime_{subc,\mu(k)}$, and $s_k^\prime$, $k\in\mathcal{K}$. The super common stream $s^\prime_{supc}$ is decoded first by treating the interference from all other streams as noise. The \gls{sinr} of the super common stream at \gls{ut}-$k$ under \gls{leo}-$m$ is
\begin{equation}\label{equ:super_common_SINR}
	\rho_{supc,k}^\prime= \frac{S_{supc,k}^\prime}{S_{subc,k}^\prime+S_{k}^\prime+I_{iL,p}^\prime+I_{oL,c}^\prime+I_{oL,p}^\prime+1},
\end{equation}
where $S_{supc,k}^\prime=|\mathbf{h}^{H}_{G,k}\mathbf{p}_{c}^\prime|^2$, $S_{subc,k}^\prime=|\mathbf{h}^{H}_{L,mk}\mathbf{p}_{subc,m}^\prime|^2$, $S_{k}^\prime=|\mathbf{h}^H_{L,mk}\mathbf{p}_{k}^\prime|^2$, $I_{iL,p}^\prime=\sum^{G_m}_{i=1,i\neq k}|\mathbf{h}^H_{L,mk}\mathbf{p}_{i}^\prime|^2$, $I_{oL,c}^\prime=\sum^M_{j=1,j\neq m}|\mathbf{h}^H_{L,jk}\mathbf{p}_{subc,j}^\prime|^2$ and $I_{oL,p}^\prime=\sum^M_{j=1,j\neq m}\sum^{G_j}_{i=1}|\mathbf{h}^H_{L,jk}\mathbf{p}_{i}|^2$.
\par Once $s^\prime_{supc}$ is decoded, its contribution to the original received signal $y_k^\prime$ is partially subtracted due to the imperfect \gls{sic}. After that, \gls{ut}-$k$ within group-$m$ decodes its sub-common stream $s_{subc,m}^{\prime}$ by treating other sub-common streams and private streams as noise. The \gls{sinr} of decoding the sub-common stream $s_{subc,m}^{\prime}$ at \gls{ut}-$k$ in \gls{leo}-$m$ is
\begin{equation}\label{equ:sub_common_SINR}
	\rho_{subc,k}^\prime= \frac{S_{subc,k}^\prime}{S_{k}^\prime+I_{iL,p}^\prime+I_{oL,c}^\prime+I_{oL,p}^\prime+\eta_{sup}^\prime S_{supc,k}^\prime+1},
\end{equation}
where $\eta_{sup}^\prime\in[0,1]$ is imperfect \gls{sic} parameter for super common stream. After removing its contribution to the received signal with imperfect \gls{sic}, \gls{ut}-$k$ decodes its private stream $s_k^{\prime}$. The sub-common streams are used to manage intra-\gls{leo} interference, since it contains parts of users' message which are served by the same \gls{leo}. Sub-common streams enable users partially decode interference and partially treat interference as noise.
The \gls{sinr} of decoding the private stream $s_k^{\prime}$ at \gls{ut}-$k$ in \gls{leo}-$m$ is
\begin{equation}\label{equ:2-layer_priv_SINR}
	\rho_{k}^\prime= \frac{S_{k}^\prime}{I_{iL,p}^\prime+I_{oL,c}^\prime+I_{oL,p}^\prime+\eta_{sup}^\prime S_{supc,k}^\prime+\eta_{sub}^\prime S_{subc,k}^\prime+1},
\end{equation}
where $\eta_{sub}^\prime\in[0,1]$ is imperfect \gls{sic} parameter for sub-common stream.
\par The corresponding achievable rates of \gls{ut}-$k$ in \gls{leo}-$m$ for the
streams $s^\prime_{supc}$, $s_{subc,m}^{\prime}$, and $s_k^{\prime}$ are $R_{supc,k}^{\prime}=\log_2{(1+\rho_{supc,k}^\prime)}$, $R_{subc,k}^{\prime}=\log_2(1+\rho_{subc,k}^\prime)$ and $R_{p,k}^\prime=\log_2(1+\rho_{k}^\prime)$. Since $s^\prime_{supc}$ and $s_{subc,m}^{\prime}$ are shared among all users and users in $\mathcal{G}_m$, the achievable common rate of $s^\prime_{supc}$ and $s_{subc,m}^{\prime}$ shall not exceed $R_{supc}^\prime=\min_{k\in\mathcal{K}}R_{supc,k}^{\prime}$ and $R_{subc,m}^\prime=\min_{k\in\mathcal{G}_m}R_{subc,k}^{\prime}$, respectively. $R_{supc}^\prime=\sum_{k\in\mathcal{K}}C_{sup,k}^\prime$ and $R_{subc,m}^\prime=\sum_{k\in\mathcal{G}_m}C_{sub,k}^\prime$, where $C_{sup,k}^\prime$ and $C_{sub,k}^\prime$ are $k$-th \gls{ut}'s portion of the common rate. The total achievable rate of \gls{ut}-$k$ is
\begin{equation}\label{equ:2-layer_totoal_rate}
	R_k^\prime=C_{sup,k}^\prime+C_{sub,k}^\prime+R_{p,k}^\prime,\ k\in\mathcal{G}_m.
\end{equation}



\subsection{Channel Model}
\subsubsection{\gls{geo} Satellite Channel}
We assume that the channel realizations between the satellite and different \gls{uts} are uncorrelated, because different \gls{uts} are often geographically separated by a certain distance. Following the literatures \cite{9257433,9844445}, the $(n,1)$-th entry of the channel between the \gls{geo} satellite and the $k$-th \gls{ut} can be written as
\begin{equation}\label{equ:GEO_channel}
	\begin{aligned}
		h_{G,nk}=\frac{\sqrt{G_{ut}G_{G}}}{4\pi\frac{d_{G,k}}{\lambda}\sqrt{\kappa T_{sys}B_w}}\chi_k^{-\frac{1}{2}}e^{-j\phi_k},
	\end{aligned}
\end{equation}
where $G_{ut}$ and $G_{G}$ are the \gls{ut} antenna gain and the antenna gain from the \gls{geo} satellite to the $k$-th \gls{ut}, respectively. $d_{G,k}$ and $\lambda$ denote the distance from the \gls{geo} satellite to \gls{ut}-$k$ and the carrier wavelength, respectively. $\kappa$ is the Boltzmann constant, $T_{sys}$ is the receiving system noise temperature and $B_w$ denotes the user link bandwidth. The large scale fading is modeled as $\chi_{k,dB}=10\log_{10}(\chi_k)$, and $\ln(\chi_{k,dB})\sim\mathcal{N}(\mu,\sigma)$. $\phi_k$ is channel phase. It is noted that different antenna feeds do not differ in their fading coefficients or phases, since the satellite antenna feed spacing is not large enough given the transmission distance and \gls{los} environment. $G_{G}$ can be further expressed as
\begin{equation}\label{equ:GEO_channel_sa_gain}
	G_{G}=G_{max}{\left[\frac{J_1(u_{nk})}{2u_{nk}}+36\frac{J_3(u_{nk})}{u_{nk}^3}\right]}^2,
\end{equation}
where $u_{nk}=2.07123\frac{\sin(\theta_{nk})}{\sin(\theta_{3dB})}$. $\theta_{nk}$ is the angle between $k$-\gls{ut} and the center of $n$-th beam with respect of the \gls{geo} satellite. $\theta_{3dB}$ denotes a 3 dB loss angle compared with the beam center. $G_{max}$ is the maximum beam gain of the beam center. $J_1$ and $J_3$ are first-kind Bessel functions with first-order and third-order, respectively.

\subsubsection{\gls{leo} Satellite Channel}
Following the literatures \cite{9110855,9419053}, the $(n,1)$-th entry of the channel model between $m$-th \gls{leo} satellite and $k$-th \gls{ut} is
\begin{subequations}\label{equ:LEO_channel}
	\begin{align}
		 & h_{L,k}=g_{k}(t,f)e^{j2\pi(f_{k}^{sat}t-f_{c}\tau_{k}^{\min})}e^{-j\phi_k},        \\
		 & g_{k}(t,f)=\sum_{l=0}^{L_k-1}g_{k,l}e^{j2\pi(f_{k,l}^{ut}t-f_{c}\tau_{k,l}^{ut})},
	\end{align}
\end{subequations}
where $f_{k}^{sat}$ and $\tau_{k}^{\min}$ are Doppler shift caused by the motion of the \gls{leo} satellite and the minimum value of the propagation delays of the $k$-th \gls{ut}, respectively. $\tau_{k}^{\min}=\min_l\{\tau_{k,l}\}$, where $\tau_{k,l}$ is the delay of the $l$-th path to \gls{ut} $k$. $g_{k}(t,f)$ is \gls{leo} satellite downlink channel gain. $L_k$ denotes the number of propagation paths of the $k$-th \gls{ut}. $f_{k,l}^{ut}$ represents the Doppler shift fot the path $l$ due to the mobility of \gls{ut} $k$, and $\tau_{k,l}^{ut}\triangleq\tau_{k,l}-\tau_k^{\min}$. $g_{k,l}$ is the complex-valued gain corresponding to path $l$ and \gls{ut} $k$ \cite{9852292}. $g_{k,l}$ follows Rician fading distribution with the Rician factor $\kappa_k$ and power
\begin{equation}\label{equ:LEO_channel_sa_gain}
	\begin{aligned}
		\gamma_k=\mathbb{E}\left\{{|g_{k,l}|}^2\right\}=\frac{\sqrt{G_{ut}G_{L}}}{4\pi\frac{d_{L,k}}{\lambda}\sqrt{\kappa T_{sys}B_w}}
	\end{aligned},
\end{equation}
where $G_{L}$ is the antenna gain of the \gls{leo} satellite.
\par We first consider a scenario with perfect \gls{csir} and perfect \gls{csit}. Then we investigate a more realistic case with perfect \gls{csir} and imperfect \gls{csit}. Due to the long propagation delay between a satellite and \gls{uts} as well as the mobility of satellites and \gls{uts}, it is difficult to obtain instantaneous \gls{csit}. %We assume imperfect \gls{csit} and perfect \gls{csir}.
Typically, imperfect \gls{csi} is modeled as a channel phase error in satellite communications, because time-varying phase variations change faster than the amplitude caused by environmental factors. The channel phase $\phi_k$ is denoted as the sum of a estimated angle, $\hat{\phi}_{k}$, and estimation error, $\tilde{\phi}_{k}$, i.e., $\phi_{k}=\hat{\phi}_{k}+\tilde{\phi}_{k}$. The angle estimation error is characterized by an uniform distribution $\tilde{\phi}_k\sim U[\phi_L,\phi_U]$.
